Weighted Null-Space Fitting for Identification of Cascade Networks

For identification of systems embedded in dynamic networks, applying the prediction error method (PEM) to a correct tailor-made parametrization of the complete network provided asymptotically efficient estimates. However, the network complexity often hinders a successful application of PEM, which requires minimizing a non-convex cost function that in general becomes more difficult for more complex networks. For this reason, identification in dynamic networks often focuses in obtaining consistent estimates of particular network modules of interest. A downside of such approaches is that splitting the network in several modules for identification often costs asymptotic efficiency. In this paper, we consider the particular case of a dynamic network with the individual systems connected in a serial cascaded manner, with measurements affected by sensor noise. We propose an algorithm that estimates all the modules in the network simultaneously without requiring the minimization of a non-convex cost function. This algorithm is an extension of Weighted Null-Space Fitting (WNSF), a weighted least-squares method that provides asymptotically efficient estimates for single-input single-output systems. We illustrate the performance of the algorithm with simulation studies, which suggest that a network WNSF may also be asymptotically efficient estimates when applied to cascade networks, and discuss the possibility of extension to more general networks affected by sensor noise.

==> conclusion.tex <==
In this paper, we proposed a method for identification of serial cascade networks. 
The method is based on WNSF, which has been shown to be asymptotically efficient for SISO models~\citep{wnsf_journal}.
The simulation study supports the idea that WNSF is also asymptotically efficient for the considered cascade networks, and the aforementioned work gives theoretical support to this idea.

For simplicity of presentation, we introduced the method for the network in Fig. 1, and discussed in Section~\ref{sec:extensions} how to extended to more generic serial cascade networks.
We pointed out that some cases require an intermediate step, which we will detail in a future contribution.
Future work will also include an extension of the method to more general network structures other than serial cascade.


==> simple_cascade.tex <==
In this section, we will use a simple cascade structure to illustrate existing identification methods for this type of network structure.
The example considered is in Fig. Y, which can be written as
\begin{equation}
\underbrace{
\begin{bmatrix}
y_1(t) \\ y_2(t)
\end{bmatrix}}_{y(t)}
=
\underbrace{
\begin{bmatrix}
G_1(q) \\
G_2(q) G_1(q)
\end{bmatrix}}_{G(q)}
u(t) +
\underbrace{
\begin{bmatrix}
e_1(t) \\ e_2(t)
\end{bmatrix}}_{e(t)}.
\label{eq:simple_cascade}
\end{equation}
As defined in Section 2, we model $G_1(q,\theta_1)$ and $G_2(q,\theta_2)$ as rational transfer functions.

\subsection{Prediction Error Method}

The idea of the prediction error method (PEM) is to minimize a cost function of the prediction errors.
For the cascade network considered in this paper, the prediction errors are given by
\begin{equation}
\varepsilon(t,\theta) = y(t) - G(q,\theta).
\end{equation}
Then, with a quadratic cost function, PEM consists of minimizing
\begin{equation}
V_N(\theta) = \det \left[ \frac{1}{N} \sum_{t=1}^N \varepsilon(t,\theta) \varepsilon^\top(t,\theta) \right],
\end{equation}
where $N$ is the sample size.

The global minimizer $\hat{\theta}_N$ of this cost function is an asymptotically efficient estimate of $\theta$ (i.e., its asymptotic covariance corresponds to the Cr{\'a}m{\'e}r-Rao bound, which is the minimum possible covariance for a consistent estimator).
The problem is that this is, in general, a non-convex cost function, for which optimization algorithms can converge to a non-global minimum.
Although this is the case also for SISO systems, the cascade case is of more concern.
First, the size of the problem increases with the number of systems in the network; second, the non-convexity cannot be solved here by using model structures such as finite impulse response (FIR) or auto-regressive with exogenous input (ARX), because of the product $G_2(q)G_1(q)$; third, methods to provide initialization points for PEM may not be directly applicable to cascade networks.

For these reasons, applying PEM to a cascade network may not always be feasiable.
We will now overview some alternative methods.

\subsection{Indirect PEM}

Indirect PEM was proposed by Soderstrom et al. to simplify, in some cases, the prediction error cost function.
The basic idea is to, in a first step, use PEM to identify an over-parametrized model that is simpler than the model of interest.
Then, in a second step, the estimated over-parametrized model is reduced to the model of interest using maximum likelihood.
This provides asymptotically efficient estimates of the model of interest.
In some cases, the over-parametrized model can be chosen such that the first step becomes a least-squares problem.
Then, the second step is typically a problem of small size which is simple to handle even if the maximum likelihood cost function is not convex.

Wahlberg et al. have observed that indirect PEM is an appropriate method to identify the cascade network~\eqref{eq:simple_cascade} if $G_1(q,\theta_1)$ and $G_2(q,\theta_2)$ are of FIR type.
However, in the case of rational transfer functions, indirect PEM does not provide an advantage with respect to PEM.

% In this case, the first step consists of identifying the model
% \begin{equation}
% \begin{bmatrix}
% y_1(t) \\ y_2(t)
% \end{bmatrix}
% =
% \begin{bmatrix}
% \tilde{G}_1(q,\theta_1) \\
% \tilde{G}_{21}(q,\theta_{21})
% \end{bmatrix}
% u(t) +
% \begin{bmatrix}
% e_1(t) \\ e_2(t)
% \end{bmatrix},
% \end{equation}
% where $\tilde{G}_1(q,\eta_1)$ has an FIR parametrization identical to $G_1(q,\theta_1)$, and $\tilde{G}_{21}(q,\eta_{21})$ has an FIR parametrization of the order of the product $G_1(q,\theta_1)G_2(q,\theta_2)$, but independent of $\tilde{G}_1(q,\eta_{21})$.
% Then, the model structure consisting of $\{\tilde{G}_1(q,\eta_1),\tilde{G}_{21}(q,\eta_{21})\}$ is over-parametrized compared to $\{G_1(q,\theta_1),G_2(q,\theta_2)\}$.
% The advantage of the over-parametrized model is that it is a SIMO FIR model, which can be estimated by least squares.

% The second step consists of using the relations
% \begin{equation}
% \left\{
% \begin{array}{l}
% G_1(q,\theta_1) = \tilde{G}_1(q,\eta_1) \\
% G_2(q,\theta_2) G_1(q,\theta_1) = \tilde{G}_{21}(q,\eta_{21}) \\
% \end{array}\right.
% \end{equation}
% and the estimates $\hat{\eta}_1$ and $\hat{\eta}_{21}$ obtained in the second step (and their covariance matrix) to obtain maximum likelihood estimates of $\theta_1$ and $\theta_2$.
% Although this is, in general, a non-convex optimization, it is typically an easy problem if $G_1(q,\theta_1)$ and $G_2(q,\theta_2)$ are of relatively low dimension.

\subsection{Over-parametrized PEM and Model Order Reduction}

In the previous approaches, simultaneous estimates of $G_1(q,\theta_1)$ and $G_2(q,\theta_2)$ were attempted to make use of all the information available.
However, because of the additional difficulty of the problem, we now consider the possibility of identifying each module separately, which does not provide asymptotically efficient estimates.

For $G_1(q,\theta_1)$, a straightforward approach is to apply PEM to the SISO model defined by the first equation in~\eqref{eq:simple_cascade}, which would provide an estimate $\hat{\theta}_1$.
Obtaining an estimating of $G_2(q,\theta_2)$ is not as straightforward: because the input to $G_2(q)$ is not known, and using $y_1(t)$ as an noisy measured input would provide biased estimates, $G_2(q,\theta_2)$ cannot be obtained directly with PEM.
One possibility is to estimate, similarly to indirect PEM but now with a rational transfer function, the over-parametrized model
\begin{equation}
y_2(t) = G_{21}(q,\theta_{21}) u(t) + e_2(t),
\end{equation}
where $G_{21}(q,\theta_{21})$ is parametrized to have the desired structure for the product $G_1(q)G_2(q)$, but with an independent parametrization of what was used for $G_1(q,\theta_1)$.
This would provide an estimate $\hat{\theta}_{21}$.

Having estimates $G_1(q,\hat{\theta}_1)$ and $G_{21}(q,\hat{\theta}_{21})$, the estimate $\hat{G}_2(q) = G_{21}(q,\hat{\theta}_{21})/G_1(q,\hat{\theta}_1)$ is an over-parametrized estimate of $G(q,\theta_2)$.
%The reason is that, due to noisy, the part of $G_{21}(q,\hat{\theta}_{21})$ that captures $G_1(q)$ will not cancel with $G_1(q,\hat{\theta}_1)$.
An estimate of $G_2(q)$ of desired order can then be obtained by performing model order reduction on $\hat{G}_2(q)$.

% Splitting the problem into two separate SISO problems is done at the cost of a loss in accuracy: the estimates obtained are in general not asymptotically efficient.
% Moreover, quantifying the uncertainty on the estimates becomes more difficult after the model reduction step.

\subsection{PEM with Simulated Data}

This approach is similar to the previous one in the sense that the model is split into two SISO models, and thus it will also not provide asymptotically efficient estimates.
However, it does not require using model order reduction.

The first step, to estimate $G_1(q,\theta_1)$, is identical.
Then, because the input to $G_2(q)$ is unknown, the idea is to simulate that input using
\begin{equation}
\hat{u}_2(t) = G_1(q,\hat{\theta}_1) u(t) ,
\end{equation}
which can then be used to estimate $G_2(q,\theta_2)$ using the data set $\{y_2(t),\hat{u}_2(t)\}$.
% Then, PEM can be applied to the SISO model
% \begin{equation}
% y_2(t) = G_2(q,\theta_2) \hat{u}_2(t) + e_2(t) .
% \end{equation}

%Despite not requiring the model order reduction step, asymptotically efficient estimates cannot be obtained with this approach for the same reason as before.

\subsection{Instrumental Variable and Subspace Methods}

Another possible approach to estimate $G_2(q,\theta_2)$ after $G_1(q,\theta_1)$ has been estimated with PEM is to use $y_2$ as a noisy input to $G_2(q)$.
This is an errors-in-variables problem, for which PEM provides biased estimates.
However, Instrumental Variable methods can be applied to this problem to obtain consistent estimates of $G_2(q,\theta_2)$.
However, asymptotically efficiency cannot be obtained.

Subspace methods that maintain the cascade structure have also been studied (Hagg et al, Wahlberg and Sandberg).
However, these approaches are limited to the simple network of Fig. 2, and have not been generalized for other cascade structures.
Moreover, subspace in general does not provide asymptotically efficient estimates.

==> tikzlibrarydsp.code.tex <==
% -------------------------------------------------------------------------
% This library for block diagrams and signal flow graphs was inspired by
% the library "signalflow" of Dr. Karlheinz Ochs, Ruhr-University of Bochum,
% Germany. Furthermore, some ideas were taken from the library "circuitikz"
% of Massimo A. Redaelli and from the PGF library itself.
%
% Copyright 2012 by Matthias Hotz
%
% This work is licensed under the Creative Commons Attribution 2.5 Generic
% License. To view a copy of this license, visit
%          http://creativecommons.org/licenses/by/2.5/
% or send a letter to Creative Commons, 444 Castro Street, Suite 900,
% Mountain View, California, 94041, USA.
% -------------------------------------------------------------------------

\usetikzlibrary{arrows, calc, positioning, decorations.markings}

% -------------------------------------------------------------------------
% Parameters for the library

\newcommand{\dsplinewidth}{0.25mm}           % Line width for connections
\newcommand{\dspblocklinewidth}{0.3mm}       % Line width for blocks
\newcommand{\dspoperatordiameter}{4mm}       % Diameter for adder, multiplier, mixer
\newcommand{\dspoperatorlabelspacing}{2mm}   % Distance from symbol to label for adder, multiplier, mixer
\newcommand{\dspnoderadius}{1mm}             % Filled and empty node
\newcommand{\dspsquareblocksize}{8mm}        % Size for square blocks, e.g. for delay elements, decimator, expander
\newcommand{\dspfilterwidth}{14mm}           % Width of a filter block

% -------------------------------------------------------------------------
% Define new arrow heads

\pgfarrowsdeclare{dsparrow}{dsparrow}
{
	\arrowsize=0.25pt
	\advance\arrowsize by .5\pgflinewidth
	\pgfarrowsleftextend{-4\arrowsize}
	\pgfarrowsrightextend{4\arrowsize}
}
{
	\arrowsize=0.25pt
	\advance\arrowsize by .5\pgflinewidth
	\pgfsetdash{}{0pt} % Solid line (do not dash)
	\pgfsetmiterjoin	 % Fixed miter join of line
	\pgfsetbuttcap		 % Fixed butt cap of line
	\pgfpathmoveto{\pgfpoint{-4\arrowsize}{2.5\arrowsize}}
	\pgfpathlineto{\pgfpoint{4\arrowsize}{0pt}}
	\pgfpathlineto{\pgfpoint{-4\arrowsize}{-2.5\arrowsize}}
	\pgfpathclose
	\pgfusepathqfill
}

\pgfarrowsdeclare{dsparrowmid}{dsparrowmid}
{
	\arrowsize=0.25pt
	\advance\arrowsize by .5\pgflinewidth
	\pgfarrowsleftextend{-4\arrowsize}
	\pgfarrowsrightextend{4\arrowsize}
}
{
	\arrowsize=0.25pt
	\advance\arrowsize by .5\pgflinewidth
	\pgfsetdash{}{0pt}
	\pgfsetmiterjoin
	\pgfsetbuttcap
	\pgfpathmoveto{\pgfpoint{0}{2.5\arrowsize}}
	\pgfpathlineto{\pgfpoint{8\arrowsize}{0pt}}
	\pgfpathlineto{\pgfpoint{0}{-2.5\arrowsize}}
	\pgfpathclose
	\pgfusepathqfill
}

% -------------------------------------------------------------------------
% Define new node shapes

\makeatletter

\pgfkeys{/tikz/dsp/label/.initial=above}

% Generic shape generator for operators, i.e. nodes with a circular
% shape with an additional customizable drawing and a text label
\long\def\dspdeclareoperator#1#2{
	\pgfdeclareshape{#1}
	{
		% Saved anchors, macros and dimensions
		\savedanchor\centerpoint{\pgfpointorigin}
		\savedmacro\label{\def\label{\pgfkeysvalueof{/tikz/dsp/label}}}
	  \saveddimen\radius
	  {
		  \pgfmathsetlength\pgf@xa{\pgfshapeminwidth}
		  \pgfmathsetlength\pgf@ya{\pgfshapeminheight}
	    \ifdim\pgf@xa>\pgf@ya
	      \pgf@x=.5\pgf@xa
	    \else
	      \pgf@x=.5\pgf@ya
	    \fi
	  }
	  
	  % Inherit all anchors from the 'circle'-shape:
	  \inheritanchor[from={circle}]{center}
	  \inheritanchor[from={circle}]{mid}
	  \inheritanchor[from={circle}]{base}
	  \inheritanchor[from={circle}]{north}
	  \inheritanchor[from={circle}]{south}
	  \inheritanchor[from={circle}]{west}
	  \inheritanchor[from={circle}]{east}
	  \inheritanchor[from={circle}]{mid west}
	  \inheritanchor[from={circle}]{mid east}
	  \inheritanchor[from={circle}]{base west}
	  \inheritanchor[from={circle}]{base east}
	  \inheritanchor[from={circle}]{north west}
	  \inheritanchor[from={circle}]{south west}
	  \inheritanchor[from={circle}]{north east}
	  \inheritanchor[from={circle}]{south east}
	  \inheritanchorborder[from={circle}]
	  
	  % Draw circle and embed additional code
	  \backgroundpath
	  {
	    % Draw circle
	    \pgfpathcircle{\centerpoint}{\radius}
	    
	    % Embed additional code
	    % (Note that this code must call e.g. \pgfusepathqstroke
	    #2
	  }
	
		% Define anchor parametrized by the PGF key /tikz/dsp/label
	  \anchor{text}
	  {
			\centerpoint
			%
	    \def\templabelabove{above}
	    \def\templabelbelow{below}
	    \def\templabelleft{left}
	    \def\templabelright{right}
	    \pgfutil@tempdima=\dspoperatorlabelspacing
	    %
	    \ifx\label\templabelabove
				\advance\pgf@x by -0.5\wd\pgfnodeparttextbox
				\advance\pgf@y by \radius
				\advance\pgf@y by \pgfutil@tempdima
	    \fi
	    %
	    \ifx\label\templabelbelow
				\advance\pgf@x by -0.5\wd\pgfnodeparttextbox
				\advance\pgf@y by -\radius
				\advance\pgf@y by -\pgfutil@tempdima
				\advance\pgf@y by -\ht\pgfnodeparttextbox
	    \fi
	    %
	    \ifx\label\templabelleft
				\advance\pgf@x by -\radius
				\advance\pgf@x by -\pgfutil@tempdima
				\advance\pgf@x by -\wd\pgfnodeparttextbox
				\advance\pgf@y by -0.5\ht\pgfnodeparttextbox
				\advance\pgf@y by +0.5\dp\pgfnodeparttextbox
	    \fi
	    %
	    \ifx\label\templabelright
				\advance\pgf@x by \radius
				\advance\pgf@x by \pgfutil@tempdima
				\advance\pgf@y by -0.5\ht\pgfnodeparttextbox
				\advance\pgf@y by +0.5\dp\pgfnodeparttextbox
	    \fi
	  }
	}
}

\dspdeclareoperator{dspshapecircle}{\pgfusepathqstroke}

\dspdeclareoperator{dspshapecirclefull}{\pgfusepathqfillstroke}

\dspdeclareoperator{dspshapeadder}{
	% Coordinate offset for the plus
	\pgfutil@tempdima=\radius
	\pgfutil@tempdima=0.55\pgfutil@tempdima
	
	% Draw plus
	\pgfmoveto{\pgfpointadd{\centerpoint}{\pgfpoint{0pt}{-\pgfutil@tempdima}}}
	\pgflineto{\pgfpointadd{\centerpoint}{\pgfpoint{0pt}{ \pgfutil@tempdima}}}
	
	\pgfmoveto{\pgfpointadd{\centerpoint}{\pgfpoint{-\pgfutil@tempdima}{0pt}}}
	\pgflineto{\pgfpointadd{\centerpoint}{\pgfpoint{ \pgfutil@tempdima}{0pt}}}
	
	\pgfusepathqstroke
}

\dspdeclareoperator{dspshapemixer}{
	% Coordinate offset for the cross
	\pgfutil@tempdima=\radius
	\pgfutil@tempdima=0.707106781\pgfutil@tempdima
	
	% Draw cross
	\pgfmoveto{\pgfpointadd{\centerpoint}{\pgfpoint{-\pgfutil@tempdima}{-\pgfutil@tempdima}}}
	\pgflineto{\pgfpointadd{\centerpoint}{\pgfpoint{ \pgfutil@tempdima}{ \pgfutil@tempdima}}}
	
	\pgfmoveto{\pgfpointadd{\centerpoint}{\pgfpoint{-\pgfutil@tempdima}{ \pgfutil@tempdima}}}
	\pgflineto{\pgfpointadd{\centerpoint}{\pgfpoint{ \pgfutil@tempdima}{-\pgfutil@tempdima}}}
	
	\pgfusepathqstroke
}

\makeatother

% -------------------------------------------------------------------------
% Define node styles

\tikzset{dspadder/.style={shape=dspshapeadder,line cap=rect,line join=rect,
	line width=\dspblocklinewidth,minimum size=\dspoperatordiameter}}
\tikzset{dspmultiplier/.style={shape=dspshapecircle,line cap=rect,line join=rect,
	line width=\dspblocklinewidth,minimum size=\dspoperatordiameter}}
\tikzset{dspmixer/.style={shape=dspshapemixer,line cap=rect,line join=rect,
	line width=\dspblocklinewidth,minimum size=\dspoperatordiameter}}

\tikzset{dspnodeopen/.style={shape=dspshapecircle,line width=\dsplinewidth,minimum size=\dspnoderadius}}
\tikzset{dspnodefull/.style={shape=dspshapecirclefull,line width=\dsplinewidth,fill,minimum size=\dspnoderadius}}

% The fixed specification of text height and text depth is the somewhat
% unaesthetic workaround to align the text in different node at the same
% baseline. See the PGF/TikZ manual, ch. 5.1.
\tikzset{dspsquare/.style={shape=rectangle,draw,align=center,text depth=0.3em,text height=1em,inner sep=0pt,
	line cap=round,line join=round,line width=\dsplinewidth,minimum size=\dspsquareblocksize}}
\tikzset{dspfilter/.style={shape=rectangle,draw,align=center,text depth=0.3em,text height=1em,inner sep=0pt,
	line cap=round,line join=round,line width=\dsplinewidth,minimum height=\dspsquareblocksize,minimum width=\dspfilterwidth}}

% -------------------------------------------------------------------------
% Define "signal flow" lines

\tikzset{dspline/.style={line width=\dsplinewidth},line cap=round,line join=round}
\tikzset{dspconn/.style={->,>=dsparrow,line width=\dsplinewidth},line cap=round,line join=round}%line cap=rect,line join=miter}
\tikzset{dspflow/.style={line width=\dsplinewidth,line cap=round,line join=round,
  decoration={markings,mark=at position 0.5 with {\arrow{dsparrowmid}}},postaction={decorate}}}

% -------------------------------------------------------------------------
% Define various utility macros

\newcommand{\downsamplertext}[1]{\raisebox{0.1em}{$\big\downarrow$}#1}
\newcommand{\upsamplertext}[1]{\raisebox{0.1em}{$\big\uparrow$}#1}

